A Framework to Quantify Approximate Simulation on Graph Data

Simulation and its variants (e.g., bisimulation and degree-preserving simulation) are useful in a wide spectrum of applications. However, all simulation variants are coarse "yes-or-no" indicators that simply confirm or refute whether one node simulates another, which limits the scope and power of their utility. Therefore, it is meaningful to develop a fractional $\chi$-simulation measure to quantify the degree to which one node simulates another by the simulation variant $\chi$. To this end, we first present several properties necessary for a fractional $\chi$-simulation measure. Then, we present $FSim_\chi$, a general fractional $\chi$-simulation computation framework that can be configured to quantify the extent of all $\chi$-simulations. Comprehensive experiments and real-world case studies show the measure to be effective and the computation framework to be efficient.

==> sec4.3_speeding_up_computation.tex <==
\stitle{Speeding Up Computation.} According to \refeq{fractional_simulation_computation}, we need to compute the scores of all node pairs in terms of iterative computation. In order to speed up the computation, we present the following two strategies to reduce the computation complexities.  

% \sstitle{Strategy 1: Shrinking candidate node pairs.} Be

\sstitle{Strategy 1: Upper-Bound Updating.} Upper-bound updating leverages the fact that there exists an upper bound of $\Sim_{\chi}(u,v)$ value for $\forall (u,v) \in V_1 \times V_2$, which is computed as follows.
\begin{equation} \label{eq:upper_bound_label_constrained_mapping}
\begin{split}
\small
    {\Sim}_\chi(u,v) &\leq  \frac{\outparam |\mathcal{M}_{\chi}(N^+(u), N^+(v))|}{\normopr_{\chi}(N^+(u), N^+(v))}
    + \frac{\inparam |\mathcal{M}_{\chi}(N^-(u), N^-(v))|}{\normopr_{\chi}(N^-(u), N^-(v))} \\&+\lparam \inifunc(u,v)
\end{split}
\end{equation}
We denote the upper bound in \refeq{upper_bound_label_constrained_mapping} as $\overline{{\Sim}_{\chi}}(u,v)$. According to C1 in \refthm{convergence}, the upper bound value should stay fixed. Given a small value $\gamma$ as threshold,  we can prune the computation of the node pairs with $\overline{{\Sim}_{\chi}}(u, v) < \gamma$, and directly use $\overline{{\Sim}_{\chi}}(u, v)$ instead if ${\Sim}_{\chi}(u, v)$ is needed during updating. By doing so, we only need to update the node pairs which are promised to be larger than $\gamma$. {\color{red}We give pseudo code in page 10}.

\sstitle{Strategy 2: Parallelization.} We utilize parallel computation as another strategy, which can speed up both the iterative computation (\refeq{fractional_simulation_computation}) and the upper-bound updating. Note that we need to deploy a hash map for the simulation scores in the previous iteration, which makes the computations of node pairs independent of each other, and can be easily parallelized. We simply round-robin the node pairs in the hash map to distribute the load to all available threads, which achieves a satisfactory scalability in the experiment (\reffig{parallelization_and_scalability}). 

